Conformal Mesh Parameterization Using Discrete Calabi Flow

In this paper, we introduce discrete Calabi flow to the graphics research community and present a novel conformal mesh parameterization algorithm. Calabi energy has a succinct and explicit format. Its corresponding flow is conformal and convergent under certain conditions. Our method is based on the Calabi energy and Calabi flow with solid theoretical and mathematical base. We demonstrate our approach on dozens of models and compare it with other related flow based methods, such as the well-known Ricci flow and CETM. Our experiments show that the performance of our algorithm is comparably the same with other methods. The discrete Calabi flow in our method provides another perspective on conformal flow and conformal parameterization.

==> experiment.tex <==
\section{Experiments}

We used calabi flow to achieve euclidean parameterization, and compare the results with discrete Ricci flow and CETM.

\subsection{Performance}

\textbf{Convergence.} In theory, if flat circle packing metric exists, then the Calabi flow will converge to that flat metric. The difference between current curvatures and target curvatures will stably descreased. But since the optimization method is first-order, so the convergence is slow.

\textbf{Conformity. }
Fig. \ref{conformaltest} is a conformality test. From the hist, We can see that most angle are perfectly preserved. And from the texture, we see that the cross angles of chessboard are preserved.

\begin{figure*}
\centering
\includegraphics[height=2in]{images/conformal_test/bunny_3D_calabi.png}
\includegraphics[height=2in]{images/conformal_test/bunny_flat_calabi.png}
\includegraphics[height=2in]{images/conformal_test/bunny26k_calabi.png}
\caption{Comformality Test. Model (26k faces, left), mapping result(middle) and angle ratio hist(right).}
\label{conformaltest}
\end{figure*}


\subsection{Comparision with Ricci Flow and CETM}
We applied Calabi flow, Ricci flow and CETM to numbers of meshes to achieve Euclidean parameterization under different boudnary settings. The texture mapping results are showed in Fig. \ref{freebound}, Fig. \ref{circlebound}, Fig. \ref{rectbound} and Fig. \ref{torus}.
Except topological tori, all models are sliced to be topoloical disks. For tori, we slice them to disks after the flow and before the embedding.

\begin{figure*}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{Calabi flow} &\multicolumn{2}{c|}{Ricci flow}&\multicolumn{2}{c|}{CETM}\\
\hline 
%\begin{sideways}Free Boundary\end{sideways}& 

\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bimba_3Duv_calabi.png}
 
& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bimba_flatuv_calabi_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bimba_3Duv_ricci.png} 

&\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bimba_flatuv_ricci_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bimba_3Duv_cetm.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bimba_flatuv_cetm_checkboard1.png}\\ 

\hline

\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bunny26k_3Duv_calabi.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bunny26k_flatuv_calabi_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bunny26k_3Duv_ricci.png} 

&\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bunny26k_flatuv_ricci_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bunny26k_3Duv_cetm.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bunny26k_flatuv_cetm_checkboard1.png}\\

\hline

\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/akitten_3Duv_calabi.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/akitten_flatuv_calabi_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/akitten_3Duv_ricci.png} 

&\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/akitten_flatuv_ricci_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/akitten_3Duv_cetm.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/akitten_flatuv_cetm_checkboard1.png}\\

\hline

\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bonefoot_3Duv_calabi.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bonefoot_flatuv_calabi_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bonefoot_3Duv_ricci.png} 

&\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bonefoot_flatuv_ricci_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bonefoot_3Duv_cetm.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/FreeBoundIMG/bonefoot_flatuv_cetm_checkboard1.png}\\

\hline

\end{tabular}

\caption{Euclidean Parametrization via Calabi flow, Ricci flow and CETM with free boundary setting. Models from up to bottom are bimba (26k faces), bunny (26k faces), kitten (9k faces) and foot bone (9k faces).}
\label{freebound}
\end{figure*}



\begin{figure*}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{Calabi flow} &\multicolumn{2}{c|}{Ricci flow}&\multicolumn{2}{c|}{CETM}\\

\hline 

\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/bimba_3Duv_calabi.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/bimba_flatuv_calabi_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/bimba_3Duv_ricci.png} 

&\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/bimba_flatuv_ricci_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/bimba_3Duv_cetm.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/bimba_flatuv_cetm_checkboard1.png}\\ 

\hline

\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/bunny26k_3Duv_calabi.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/bunny26k_flatuv_calabi_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/bunny26k_3Duv_ricci.png} 

&\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/bunny26k_flatuv_ricci_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/bunny26k_3Duv_cetm.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/bunny26k_flatuv_cetm_checkboard1.png}\\ 

\hline

\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/mug_3Duv_calabi.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/mug_flatuv_calabi_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/mug_3Duv_ricci.png} 

&\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/mug_flatuv_ricci_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/mug_3Duv_cetm.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/mug_flatuv_cetm_checkboard1.png}\\ 

\hline

\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/eight_3Duv_calabi.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/eight_flatuv_calabi_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/eight_3Duv_ricci.png} 

&\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/eight_flatuv_ricci_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/eight_3Duv_cetm.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/CircleIMG/eight_flatuv_cetm_checkboard1.png}\\ 

\hline

\end{tabular}
\caption{Euclidean Parametrization via Calabi flow, Ricci flow and CETM with circlular boundary setting. Models from up to bottom are bimba (26k faces), bunny (26k faces), mug (9k faces) and eight (7k faces).}
\label{circlebound}
\end{figure*}

\begin{figure*}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{Calabi flow} &\multicolumn{2}{c|}{Ricci flow}&\multicolumn{2}{c|}{CETM}\\

\hline 

\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/antdisk_3Duv_calabi.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/antdisk_flatuv_calabi_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/antdisk_3Duv_ricci.png} 

&\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/antdisk_flatuv_ricci_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/antdisk_3Duv_cetm.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/antdisk_flatuv_cetm_checkboard1.png}\\ 

\hline 

\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/bunny26k_3Duv_calabi.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/bunny26k_flatuv_calabi_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/bunny26k_3Duv_ricci.png} 

&\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/bunny26k_flatuv_ricci_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/bunny26k_3Duv_cetm.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/bunny26k_flatuv_cetm_checkboard1.png}\\ 

\hline

\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/mug_3Duv_calabi.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/mug_flatuv_calabi_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/mug_3Duv_ricci.png} 

&\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/mug_flatuv_ricci_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/mug_3Duv_cetm.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/mug_flatuv_cetm_checkboard1.png}\\ 

\hline

\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/eight_3Duv_calabi.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/eight_flatuv_calabi_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/eight_3Duv_ricci.png} 

&\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/eight_flatuv_ricci_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/eight_3Duv_cetm.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/RectIMG/eight_flatuv_cetm_checkboard1.png}\\ 

\hline

\end{tabular}
\caption{Euclidean Parametrization via Calabi flow, Ricci flow and CETM with circlular boundary setting. Models from up to bottom are ant (11k faces), bunny (26k faces), mug (9k faces) and eight (7k faces).}
\label{rectbound}
\end{figure*}


\begin{figure*}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{Calabi flow} &\multicolumn{2}{c|}{Ricci flow}&\multicolumn{2}{c|}{CETM}\\

\hline 

\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/TorusIMG/akitten_3Duv_calabi.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/TorusIMG/akitten_flatuv_calabi_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/TorusIMG/akitten_3Duv_ricci.png} 

&\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/TorusIMG/akitten_flatuv_ricci_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/TorusIMG/akitten_3Duv_cetm.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/TorusIMG/akitten_flatuv_cetm_checkboard1.png}\\ 

\hline

\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/TorusIMG/vase2_3Duv_calabi.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/TorusIMG/vase2_flatuv_calabi_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/TorusIMG/vase2_3Duv_ricci.png} 

&\includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/TorusIMG/vase2_flatuv_ricci_checkboard1.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/TorusIMG/vase2_3Duv_cetm.png} 

& \includegraphics[width = 1.0in]{images/Euclidean_Experiment_Result/TorusIMG/vase2_flatuv_cetm_checkboard1.png}\\ 

\hline

\end{tabular}
\caption{Euclidean Parametrization via Calabi flow, Ricci flow and CETM for genus one closed surface. Models from up to bottom are kitten (9k faces) and vase (k faces).}
\label{torus}
\end{figure*}



1.  we compare the mesh parameterization result with Ricci flow and CETM. The experiments shows that: 







2.  we compare three algorithms in hundreds of models, The following table shows their conformity:





3. in this figure, we show................



\textbf{Analysis and Comparison } 
According to our experiments, the three algorithms ........


